Neurosymbolic AI for Reasoning over Knowledge Graphs: A Survey

Neurosymbolic AI is an increasingly active area of research that combines symbolic reasoning methods with deep learning to leverage their complementary benefits. As knowledge graphs are becoming a popular way to represent heterogeneous and multi-relational data, methods for reasoning on graph structures have attempted to follow this neurosymbolic paradigm. Traditionally, such approaches have utilized either rule-based inference or generated representative numerical embeddings from which patterns could be extracted. However, several recent studies have attempted to bridge this dichotomy to generate models that facilitate interpretability, maintain competitive performance, and integrate expert knowledge. Therefore, we survey methods that perform neurosymbolic reasoning tasks on knowledge graphs and propose a novel taxonomy by which we can classify them. Specifically, we propose three major categories: (1) logically-informed embedding approaches, (2) embedding approaches with logical constraints, and (3) rule learning approaches. Alongside the taxonomy, we provide a tabular overview of the approaches and links to their source code, if available, for more direct comparison. Finally, we discuss the unique characteristics and limitations of these methods, then propose several prospective directions toward which this field of research could evolve.

==> archive/rebuttal.tex <==


BEGINNING OF COMMENTS TO THE AUTHOR(S)
+++++++++++++++++++++++++++++++++++++++

Recommended Decision by Associate Editor: Recommendation #1: Reject & Resubmit

Recommendation #2: Reject & Resubmit

Comments to Author(s) by Associate Editor:
Senior Editor: 1
Comments to the Author:
In addition, the paper needs to seriously address the concern on the completeness of literature review of the related subjects and the concern on its suitability for the journal - has TNNLS ever published a single paper on the topic described in this manuscript before?  If yes, why there is little mentioning of such work(s) throughout the entire manuscript? if no, then why this type of topic would be of interest to the readers of the journal? This further creates the concern on the suitability of the paper for the journal.

Associate Editor: 2
Comments to the Author:
The authors provide a survey of neurosymbolic works for KG reasoning (eg, link prediction). There is a consensus among reviewers that the taxonomy presented in the paper is meaningful, and that the figures and the text help a reader navigate the field. However, the reviewers are also raising some concerns, in particular on the distinction between "neurosymbolic" as used here and standard KG embeddings or GNNs applied to KGs. In addition, some suggestions are provided to refine the text and clarify some ideas.

+++++++++++++++++++++

Individual Reviews:

Reviewer(s)' Comments to Author(s):

Reviewer: 1

Comments to the Author
The present paper provides a review of neuro-symbolic integration approaches for knowledge graphs. The review sorts the existing methods into three categories: 1. logically-informed embeddings which first apply logical inference, followed by a knowledge graph embedding, 2. logical constraints, which constrain the learned embedding with logical rules, and 3. learning logical rules, which try to learn weights for existing rules or learn entirely new logical rules via neural approaches. Within each category, the review discusses example approaches and subdivides them according to their methodology. Figure 1 provides a taxonomy, Table 1 a tabular overview. Section V identifies gaps in the existing literature and potential directions for future work.

The main strengths of the paper are:
* The suggested taxonomy is convincing to me and the tabular overview is very helpful.
* The literature overview appears complete (at least, I do not see any obvious omissions or gaps)
* The contributions of the paper/the difference from prior reviews is reasonably clear.
* The high-level explanations of all approaches are reasonably easy to follow and provide a rough impression of all methods.
* The directions of future work follow logically from the prior discussion of literature.

Nonetheless, I also see some room for improvement:
* As it stands, the paper's focus topic appears rather niche. I believe that more motivation for neuro-symbolic approaches over knowledge graphs in the introduction is needed. In particular: Which practical challenges can be addressed by such approaches which are not already covered by purely neural or purely logical approaches? How do neuro-symbolic approaches discussed in this paper differ from simple graph embeddings/graph neural nets?
* While both taxonomy and tabular overview appear convincing to me, I do not think that the text reflects the structure with the same clarity. I would recommend to revise the text to provide a clearer narrative thread and orient the reader within the overarching taxonomy. Each section should start with: Where in the taxonomy are we now? What are the crucial characteristics of this part of the taxonomy that delineate these approaches from the others?
* I could parse Figures 2, 6, and 8, but I am not convinced that Figures 3, 4, 5, or 7 contribute much to understanding. In more detail: The arrows in the center of Fig. 3 are unclear to me. How do logical inference and KG embeddings interact? In Fig. 4 I do not think that the 'constraints' arrow tells me much about how constraints act on the embedding. The same applies for the arrow in Figure 5. In Figure 7, I do not understand how logical inference relates to the M step and how graph decoding/embedding relates to the E-step. Could these Figures perhaps be revised to enhance clarity/understanding? Would it be possible to provide examples?
* I am not entirely convinced that the paper goes sufficiently deep in describing the different classes of approaches. There is hardly any formalization or specific examples given to provide deep understanding.

Beyond these major points, I also see some minor issues:

* When describing neural nets in section II.C or graph neural nets later on it is not sufficiently clear how the neural net approaches for knowledge graphs differ from neural nets on general graphs. Is there anything special about knowledge graphs, in this context?
* Page 2, left column, line 30 could be read as Google having invented knowledge graphs, which is certainly not the case. I recommend to adjust the phrasing to avoid this impression.
* In the review of neuro-symbolic AI, it may also be useful to cite other reviews of this field, such as Hitzler et al. (2022; https://doi.org/10.1093/nsr/nwac035 )
* page 12, left column: Are the algorithms in IV.C.1 really EM algorithms in the strict sense of Dempster, Laird, and Rubin (1977; https://www.jstor.org/stable/2984875 )? To me, it reads like the approaches are merely using some alternating optimization, but do not follow a strict probabilistic framework as required for proper EM.

Overall, I do believe that the review is solid work. However, I also think that some motivation, structure, and depth is missing.

Reviewer: 2

Comments to the Author
The manuscript surveyed a breadth of methods that perform neurosymbolic reasoning tasks on graph structures. This topic is much interesting. Some weaknesses of the manuscript are listed below.

       The survey is conducted from the perspective of neurosymbolic AI on knowledge graph complement（KGC）. However, this interesting viewpoint seems just only a superficial word to carry out a survey of knowledge graph representation learning rather than an insightful deep understanding of the integration of symbolic and neurocomputing for knowledge graph. For example, one of the benefits of neurosymbolic AI is the human-level interpretability. The manuscript lacks comprehensively discussions on how and why this benefit would happened qualitatively and quantitatively in the context of knowledge graph complement. Another example, there is no explicit discussions on whether the neurosymbolic method would help the KGC to train on less data, which is regarded as also a general benefit of neurosymbolic AI. As the results, the novelty of this survey is limited, and it is hard to distinguish this survey from previous review works on knowledge graph representation learning. The survey payed much attentions to the trivial details of KGC algorithms. In my personal opinion, unique insight and analysis of the neurosymbolic ideas behind these algorithms are more expected. Meanwhile, the potential limitations of using neurosymbolic method for KGC is also interesting topic.
       Does the word “graph” in title of this paper merely refer to the “knowledge graph”? Is there any other kind of graph reasoning task which integrates the neurosymbolic approach?
       In section II.D,  6 types of neurosymbolic integration approaches following the reference[129] was presented. However, when applied to the context of graph reasoning, only parts of the 6 types were considered and there is no discussion about the potential reasons.
       The organization of the manuscript needs polish to focus on the “Neurosymbolic” discussion rather than KGC.


Reviewer: 3

Comments to the Author
Summary)
The work is well structured and seems comprehensive.
Each section also has a figure explaining the method, which is a great addition.



Main concerns:
If I had to find a problem with this survey, I would say that, although present in the text, the "general understanding of each category's benefits and weaknesses" (Page15-Lines8-9, Right column) is not clear.
A table defining schematically these, in relation to the various categories, and possible fields of application would make the paper more complete.



Minor concerns:

Missing references)
Here is a list of lines where a reference is needed.
P1-L45-51-Left) …
P6-L34-38-Right) “Because research … for growth”


P2-L22-23-Left) Missing u, v definition (\in V)

P3-L42-45-Right) This sentence seems disconnected from the rest of the section and lacks citation. I would delete it.

P4-L11-12-Left) Actually, that’s “Deep Neural Network” or “Deep Learning models”. “Deep Learning” is a broader term.

P4-L11-12-Left) I think “superhuman” is an exaggeration and not actually proven in the cited papers

P6-L32-Left) "an entity or node type a node may be categorized” probably an error


+++++++++++++++++++++++++++++++++++++++
END OF COMMENTS TO THE AUTHOR(S)

==> sections/5_applications/5_applications.tex <==
\noindent Within the previous sections, much of the discussion around the benefits and drawbacks of each method centres around the degree of interpretability and incorporation of domain-specific knowledge that the method affords. However, the importance of these features varies with respect to the application domain on which a researcher wishes to work. As previously mentioned in section \ref{subsection:embedding_kg_completion}, domains which are relevant to peoples' health and lives, such as biomedicine, might benefit from increased interpretability for ethical reasons. For other fields, however, interpretability may not be useful \cite{molnar2022, jose2021fairness}. Furthermore, the level of available expert knowledge varies drastically between fields, and one must consider whether adding such knowledge would also add bias, such as decisions based on sensitive demographic features like ethnicity \cite{jose2021fairness}. In this brief section, we highlight and discuss the major application domains for which the surveyed methods were used in order to identify key areas in which these methods are deemed potentially useful.

The selection of application domains chosen in the surveyed papers was largely driven by a preference for commonly used and openly available KGs. For example, because they are popular benchmark datasets \cite{dai2020survey}, several KGs which encompass general knowledge bases, including YAGO \cite{suchanek2007yago}, Freebase \cite{bollacker2008freebase}, Wikidata \cite{vrandevcic2014wikidata}, and DBPedia \cite{auer2007dbpedia} were frequent choices with which to test the novel methods. WordNet \cite{miller1995wordnet}, a lexical KG of the English language, is also a well-established benchmark dataset and was also, therefore, a popular choice for testing. The use of these popular benchmark datasets explains why the \textit{General Knowledge} and \textit{Lexical Semantics} sections contain some of the most use cases, as shown in figure \ref{applications}.

This pattern is also apparent within the \textit{Social Relationship Understanding} and \textit{Biomedical} sections of figure \ref{applications}. Within the former, all approaches listed utilize the Kinship KG \cite{hinton1986learning, quinlan1989learning}, and in the latter, most approaches use a KG containing information from the unified medical language system (UMLS) \cite{bodenreider2004unified}. A handful of approaches in the \textit{Biomedical} section, however, deviate from this trend, having used a disease-specific \cite{zhao2020biomedical} or pharmaco-oriented \cite{drance2021neuro} KG to achieve more specific goals. These and several others \cite{agibetov2018fast, liu2021neural, alshahrani2017neuro} verify that these neurosymbolic methods for graph reasoning may be particularly interesting and useful within the biomedical domain.

Aside from those four major categories, we can see that there are a handful of studies which operate on other applications such as question-answering \cite{yang2017differentiable} and recommender systems \cite{HChenGCR}. However, these studies seem to be the exceptions. In general, it seems that most studies chose benchmark datasets on which to test their methods rather than KGs corresponding to domains in which they suspected their method to be useful. Future studies for neurosymbolic graph reasoning methods, could, therefore, adopt a stronger emphasis on some domain-specific use, a prospective direction discussed within the next section.

\begin{figure*}[!t]
    \centering
    \includegraphics[width=5in]{applications}
    \caption{The surveyed approaches grouped by application area and colour-coded by hierarchical section.}
    \label{applications}
\end{figure*}

